Reconstruction of 400 GeV/c proton interactions with the SHiP-charm project

The SHiP-charm project was proposed to measure the associated charm production induced by 400 GeV/c protons in a thick target, including the contribution from cascade production. An optimisation run was performed in July 2018 at CERN SPS using a hybrid setup. The high resolution of nuclear emulsions acting as vertex detector was complemented by electronic detectors for kinematic measurements and muon identification. Here we present first results on the analysis of nuclear emulsions exposed in the 2018 run, which prove the capability of reconstructing proton interaction vertices in a harsh environment, where the signal is largely dominated by secondary particles produced in hadronic and electromagnetic showers within the lead target.

==> authorlist_26august2023.tex <==
%\documentclass{article}
%\usepackage[utf8]{inputenc}
%\begin{document}
\onecolumn
%
\noindent
\textbf{The SHiP Collaboration}
\\
%\centerline{\Large\bf The SHiP Collaboration}
%\vspace*{1mm}
%\begin{flushleft}
%-- 
%-- SHiP Authorlist as of 26 August 2023
%-- 
\noindent
C.~Ahdida$^{32}$,
A.~Akmete$^{10}$,
R.~Albanese$^{15,d,h}$,
J.~Alt$^{7}$,
A.~Alexandrov$^{15,d}$,
S.~Aoki$^{18}$,
G.~Arduini$^{32}$,
J.J.~Back$^{42}$,
F.~Baaltasar~Dos~Santos$^{32}$,
F.~Bardou$^{32}$,
G.J.~Barker$^{42}$,
M.~Battistin$^{32}$,
J.~Bauche$^{32}$,
A.~Bay$^{34}$,
V.~Bayliss$^{39}$,
C.~Betancourt$^{35}$,
I.~Bezshyiko$^{35}$,
O.~Bezshyyko$^{43}$,
D.~Bick$^{8}$,
S.~Bieschke$^{8}$,
A.~Blanco$^{28}$,
J.~Boehm$^{39}$,
M.~Bogomilov$^{1}$,
I.~Boiarska$^{3}$,
K.~Bondarenko$^{27,57}$,
W.M.~Bonivento$^{14}$,
J.~Borburgh$^{32}$,
A.~Boyarsky$^{27,43}$,
R.~Brenner$^{31}$,
D.~Breton$^{4}$,
A. Brignoli$^{6}$,
V.~B\"{u}scher$^{10}$,
A.~Buonaura$^{35}$,
S.~Buontempo$^{15}$,
S.~Cadeddu$^{14}$,
M.~Calviani$^{32}$,
M.~Campanelli$^{41}$,
M.~Casolino$^{32}$,
N.~Charitonidis$^{32}$,
P.~Chau$^{10}$,
J.~Chauveau$^{5}$,
K.-Y.~Choi$^{26}$,
A.~Chumakov$^{2}$,
V.~Cicero$^{13}$,
M.~Climescu$^{10}$,
A.~Conaboy$^{6}$,
L.~Congedo$^{12,a}$,
K.~Cornelis$^{32}$,
M.~Cristinziani$^{11}$,
A.~Crupano$^{13}$,
G.M.~Dallavalle$^{13}$,
A.~Datwyler$^{35}$,
N.~D'Ambrosio$^{16}$,
G.~D'Appollonio$^{14,c}$,
R.~de~Asmundis$^{15}$,
J.~De~Carvalho~Saraiva$^{28}$,
G.~De~Lellis$^{15,32,d}$,
M.~de~Magistris$^{15,l}$,
A.~De~Roeck$^{32}$,
M.~De~Serio$^{12,a}$,
D.~De~Simone$^{35}$,
A.~Di~Crescenzo$^{15,32,d}$,
L.~Di~Giulio$^{32}$,
C.~Dib$^{2}$,
H.~Dijkstra$^{32}$,
L.A.~Dougherty$^{32}$,
V.~Drohan$^{43}$,
A.~Dubreuil$^{33}$,
O.~Durhan$^{36}$,
M.~Ehlert$^{6}$,
E.~Elikkaya$^{36}$,
F.~Fabbri$^{13}$,
F.~Fedotovs$^{40}$,
M.~Ferrillo$^{35}$,
M.~Ferro-Luzzi$^{32}$,
R.A.~Fini$^{12}$,
H.~Fischer$^{7}$,
P.~Fonte$^{28}$,
C.~Franco$^{28}$,
M.~Fraser$^{32}$,
R.~Fresa$^{15,i,h}$,
R.~Froeschl$^{32}$,
T.~Fukuda$^{19}$,
G.~Galati$^{12,a}$,
J.~Gall$^{32}$,
L.~Gatignon$^{32}$,
V.~Gentile$^{15,d}$,
B.~Goddard$^{32}$,
L.~Golinka-Bezshyyko$^{43}$,
A.~Golovatiuk$^{15,d}$,
A.~Golutvin$^{40}$,
P.~Gorbounov$^{32}$,
V.~Gorkavenko$^{43}$,
A.L.~Grandchamp$^{34}$,
E.~Graverini$^{34}$,
J.-L.~Grenard$^{32}$,
D.~Grenier$^{32}$,
A.~M.~Guler$^{36}$,
G.J.~Haefeli$^{34}$,
C.~Hagner$^{8}$,
H.~Hakobyan$^{2}$,
I.W.~Harris$^{34}$,
E.~van~Herwijnen$^{32}$,
C.~Hessler$^{32}$,
A.~Hollnagel$^{10}$,
B.~Hosseini$^{40}$,
G.~Iaselli$^{12,a}$,
A.~Iuliano$^{15,d}$,
R.~Jacobsson$^{32}$,
D.~Jokovi\'{c}$^{29}$,
M.~Jonker$^{32}$,
I.~Kadenko$^{43}$,
V.~Kain$^{32}$,
B.~Kaiser$^{8}$,
C.~Kamiscioglu$^{37}$,
K.~Kershaw$^{32}$,
G.~Khoriauli$^{10}$,
Y.G.~Kim$^{23}$,
N.~Kitagawa$^{19}$,
J.-W.~Ko$^{22}$,
K.~Kodama$^{17}$,
D.I.~Kolev$^{1}$,
M.~Komatsu$^{19}$,
A.~Kono$^{21}$,
S.~Kormannshaus$^{10}$,
I.~Korol$^{6}$,
A.~Korzenev$^{33}$,
V.~Kostyukhin$^{11}$,
E.~Koukovini~Platia$^{32}$,
S.~Kovalenko$^{2}$,
H.M.~Lacker$^{6}$,
M.~Lamont$^{32}$,
O.~Lantwin$^{15}$,
A.~Lauria$^{15,d}$,
K.S.~Lee$^{25}$,
K.Y.~Lee$^{22}$,
N.~Leonardo$^{28}$,
J.-M.~L\'{e}vy$^{5}$,
V.P.~Loschiavo$^{15,h}$,
L.~Lopes$^{28}$,
E.~Lopez~Sola$^{32}$,
F.~Lyons$^{7}$,
V.~Lyubovitskij$^{2}$,
J.~Maalmi$^{4}$,
A.-M.~Magnan$^{40}$,
Y.~Manabe$^{19}$,
M.~Manfredi$^{32}$,
S.~Marsh$^{32}$,
A.M.~Marshall$^{38}$,
P.~Mermod$^{33}$,
A.~Miano$^{15,d}$,
S.~Mikado$^{20}$,
A.~Mikulenko$^{27}$,
D.A.~Milstead$^{30}$,
A.~Montanari$^{13}$,
M.C.~Montesi$^{15,d}$,
K.~Morishima$^{19}$,
Y.~Muttoni$^{32}$,
N.~Naganawa$^{19}$,
M.~Nakamura$^{19}$,
T.~Nakano$^{19}$,
P.~Ninin$^{32}$,
A.~Nishio$^{19}$,
S.~Ogawa$^{21}$,
J.~Osborne$^{32}$,
M.~Ovchynnikov$^{27,43}$,
N.~Owtscharenko$^{11}$,
P.H.~Owen$^{35}$,
P.~Pacholek$^{32}$,
B.D.~Park$^{22}$,
A.~Pastore$^{12}$,
M.~Patel$^{40}$,
A.~Perillo-Marcone$^{32}$,
G.L.~Petkov$^{1}$,
K.~Petridis$^{38}$,
J.~Prieto~Prieto$^{32}$,
A.~Prota$^{15,d}$,
A.~Quercia$^{15,d}$,
A.~Rademakers$^{32}$,
A.~Rakai$^{32}$,
T.~Rawlings$^{39}$,
F.~Redi$^{34}$,
A.~Reghunath$^{6}$,
S.~Ricciardi$^{39}$,
M.~Rinaldesi$^{32}$,
Volodymyr~Rodin$^{43}$,
Viktor~Rodin$^{43}$,
P.~Robbe$^{4}$,
A.B.~Rodrigues~Cavalcante$^{34}$,
H.~Rokujo$^{19}$,
G.~Rosa$^{15,d}$,
T.~Rovelli$^{13,b}$,
O.~Ruchayskiy$^{3}$,
T.~Ruf$^{32}$,
F.~Sanchez~Galan$^{32}$,
P.~Santos~Diaz$^{32}$,
A.~Sanz~Ull$^{32}$,
O.~Sato$^{19}$,
J.S.~Schliwinski$^{6}$,
W.~Schmidt-Parzefall$^{8}$,
M.~Schumann$^{7}$,
N.~Serra$^{35}$,
S.~Sgobba$^{32}$,
O.~Shadura$^{43}$,
M.~Shaposhnikov$^{34}$,
L.~Shchutska$^{34}$,
H.~Shibuya$^{21}$,
L.~Shihora$^{6}$,
S.~Shirobokov$^{40}$,
S.B.~Silverstein$^{30}$,
S.~Simone$^{12,a}$,
R.~Simoniello$^{10}$,
G.~Soares$^{28}$, 
J.Y.~Sohn$^{22}$,
A.~Sokolenko$^{43}$,
E.~Solodko$^{32}$,
L.~Stoel$^{32}$,
M.E.~Stramaglia$^{34}$,
D.~Sukhonos$^{32}$,
Y.~Suzuki$^{19}$,
S.~Takahashi$^{18}$,
J.L.~Tastet$^{3}$,
I.~Timiryasov$^{34}$,
V.~Tioukov$^{15}$,
D.~Tommasini$^{32}$,
M.~Torii$^{19}$,
N.~Tosi$^{13}$,
D.~Treille$^{32}$,
R.~Tsenov$^{1}$,
G.~Vankova-Kirilova$^{1}$,
F.~Vannucci$^{5}$,
P.~Venkova$^{6}$,
V.~Venturi$^{32}$,
S.~Vilchinski$^{43}$,
Heinz~Vincke$^{32}$,
Helmut~Vincke$^{32}$,
C.~Visone$^{15,d}$,
S.~van~Waasen$^{9}$,
R.~Wanke$^{10}$,
P.~Wertelaers$^{32}$,
O.~Williams$^{32}$,
J.-K.~Woo$^{24}$,
M.~Wurm$^{10}$,
S.~Xella$^{3}$,
D.~Yilmaz$^{37}$,
A.U.~Yilmazer$^{37}$,
C.S.~Yoon$^{22}$,
J.~Zimmerman$^{6}
\vspace*{1cm}

{\footnotesize \it

$^{1}$Faculty of Physics, Sofia University, Sofia, Bulgaria\\
$^{2}$Universidad T\'ecnica Federico Santa Mar\'ia and Centro Cient\'ifico Tecnol\'ogico de Valpara\'iso, Valpara\'iso, Chile\\
$^{3}$Niels Bohr Institute, University of Copenhagen, Copenhagen, Denmark\\
$^{4}$LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit\'{e} Paris-Saclay, Orsay, France\\
$^{5}$LPNHE, IN2P3/CNRS, Sorbonne Universit\'{e}, Universit\'{e} Paris Diderot,F-73939 Paris, France\\
$^{6}$Humboldt-Universit\"{a}t zu Berlin, Berlin, Germany\\
$^{7}$Physikalisches Institut, Universit\"{a}t Freiburg, Freiburg, Germany\\
$^{8}$Universit\"{a}t Hamburg, Hamburg, Germany\\
$^{9}$Forschungszentrum J\"{u}lich GmbH (KFA),  J\"{u}lich , Germany\\
$^{10}$Institut f\"{u}r Physik and PRISMA Cluster of Excellence, Johannes Gutenberg Universit\"{a}t Mainz, Mainz, Germany\\
$^{11}$Universit\"{a}t Siegen, Siegen, Germany\\
$^{12}$Sezione INFN di Bari, Bari, Italy\\
$^{13}$Sezione INFN di Bologna, Bologna, Italy\\
$^{14}$Sezione INFN di Cagliari, Cagliari, Italy\\
$^{15}$Sezione INFN di Napoli, Napoli, Italy\\
$^{16}$Laboratori Nazionali dell'INFN di Gran Sasso, L'Aquila, Italy\\
$^{17}$Aichi University of Education, Kariya, Japan\\
$^{18}$Kobe University, Kobe, Japan\\
$^{19}$Nagoya University, Nagoya, Japan\\
$^{20}$College of Industrial Technology, Nihon University, Narashino, Japan\\
$^{21}$Toho University, Funabashi, Chiba, Japan\\
$^{22}$Physics Education Department \& RINS, Gyeongsang National University, Jinju, Korea\\
$^{23}$Gwangju National University of Education~$^{e}$, Gwangju, Korea\\
$^{24}$Jeju National University~$^{e}$, Jeju, Korea\\
$^{25}$Korea University, Seoul, Korea\\
$^{26}$Sungkyunkwan University~$^{e}$, Suwon-si, Gyeong Gi-do, Korea\\
$^{27}$University of Leiden, Leiden, The Netherlands\\
$^{28}$LIP, Laboratory of Instrumentation and Experimental Particle Physics, Portugal\\
$^{29}$Institute of Physics, University of Belgrade, Serbia\\
$^{30}$Stockholm University, Stockholm, Sweden\\
$^{31}$Uppsala University, Uppsala, Sweden\\
$^{32}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$^{33}$University of Geneva, Geneva, Switzerland\\
$^{34}$\'{E}cole Polytechnique F\'{e}d\'{e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$^{35}$Physik-Institut, Universit\"{a}t Z\"{u}rich, Z\"{u}rich, Switzerland\\
$^{36}$Middle East Technical University (METU), Ankara, Turkey\\
$^{37}$Ankara University, Ankara, Turkey\\
$^{38}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom \\
$^{39}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{40}$Imperial College London, London, United Kingdom\\
$^{41}$University College London, London, United Kingdom\\
$^{42}$University of Warwick, Warwick, United Kingdom\\
$^{43}$Taras Shevchenko National University of Kyiv, Kyiv, Ukraine\\
$^{a}$Universit\`{a} di Bari, Bari, Italy\\
$^{b}$Universit\`{a} di Bologna, Bologna, Italy\\
$^{c}$Universit\`{a} di Cagliari, Cagliari, Italy\\
$^{d}$Universit\`{a} di Napoli ``Federico II``, Napoli, Italy\\
$^{e}$Associated to Gyeongsang National University, Jinju, Korea\\
$^{f}$Associated to Petersburg Nuclear Physics Institute (PNPI), Gatchina, Russia\\
$^{g}$Also at Moscow Institute of Physics and Technology (MIPT),  Moscow Region, Russia\\
$^{h}$Consorzio CREATE, Napoli, Italy\\
$^{i}$Universit\`{a} della Basilicata, Potenza, Italy\\
$^{l}$Universit\`{a} di Napoli Parthenope, Napoli, Italy\\
}

Following the resolution of the CERN Council, Russian groups participating in the
SHiP project are not included in the author list of this document. We acknowledge the
contribution of the Russian scientists, in particular A.~Anokhina, E.~Atkin, N.~Azorskiy, A.~Bagulya, A.~Baranov, A.Y.~Berdnikov, Y.A.~Berdnikov, A.~Chepurnov, M.~Chernyavskiy, L.~Dedenko, P.~Dergachev, V.~Dmitrenko, A.~Dolmatov, S.~Donskov, T.~Enik, A.~Etenko, O.~Fedin, K.~Filippov, G.~Gavrilov, V.~Golovtsov, D.~Golubkov, D.~Gorbunov, S.~Gorbunov, M.~Gorshenkov, V.~Grachev, V.~Grichine, N.~Gruzinskii, Yu.~Guz, M.~Hushchyn, D.~Karpenkov, M.~Khabibullin, E.~Khalikov, G.~Khaustov, A.~Khotyantsev, V.~Kim, A.~Kolesnikov, V.~Kolosov, N.~Konovalova, I.~Korol'ko, I.~Krasilnikova, Y.~Kudenko, E.~Kurbatov, P.~Kurbatov, V.~Kurochka, E.~Kuznetsova, V.~Maleev, A.~Malinin, A.K.~Managadze, A.~Mefodev, Yu.~Mikhaylov, O.~Mineev, S.~Movchan, S.~Nasybulin, B.~Obinyakov, N.~Okateva, D.~Pereyma, A.~Petrov, D.~Podgrudkov, V.~Poliakov, N.~Polukhina, M.~Prokudin, F.~Ratnikov, T.~Roganova, V.~Samoylenko, V.~Samsonov, E.S.~Savchenko, A.~Shakin, P.~Shatalov, T.~Shchedrina, V.~Shevchenko, A.~Shustov, M.~Skorokhvatov, S.~Smirnov, N.~Starkov, P.~Teterin, S.~Than~Naing, S.~Ulin, E.~Ursov, A.~Ustyuzhanin, Z.~Uteshev, L.~Uvarov, I.~Vidulin, K.~Vlasik, A.~Volkov, R.~Voronkov, Yu.~Zaytsev, A.~Zelenov. 


% \end{flushleft}




% \end{document}

==> authorlist_4july2022.tex <==
%\documentclass{article}
%\usepackage[utf8]{inputenc}
%\begin{document}
\onecolumn
%
\noindent
\textbf{The SHiP Collaboration}
\\
%\centerline{\Large\bf The SHiP Collaboration}
%\vspace*{1mm}
%\begin{flushleft}
%-- 
%-- SHiP Authorlist as of 3 December 2021
%-- 
\noindent
C.~Ahdida$^{44}$,
A.~Akmete$^{10}$,
R.~Albanese$^{15,d,h}$,
J.~Alt$^{7}$,
A.~Alexandrov$^{15,32,34,d}$,
A.~Anokhina$^{39}$,
S.~Aoki$^{18}$,
G.~Arduini$^{44}$,
E.~Atkin$^{38}$,
N.~Azorskiy$^{29}$,
J.J.~Back$^{54}$,
A.~Bagulya$^{32}$,
F.~Baaltasar~Dos~Santos$^{44}$,
A.~Baranov$^{40}$,
F.~Bardou$^{44}$,
G.J.~Barker$^{54}$,
M.~Battistin$^{44}$,
J.~Bauche$^{44}$,
A.~Bay$^{46}$,
V.~Bayliss$^{51}$,
A.Y.~Berdnikov$^{37}$,
Y.A.~Berdnikov$^{37}$,
C.~Betancourt$^{47}$,
I.~Bezshyiko$^{47}$,
O.~Bezshyyko$^{55}$,
D.~Bick$^{8}$,
S.~Bieschke$^{8}$,
A.~Blanco$^{28}$,
J.~Boehm$^{51}$,
M.~Bogomilov$^{1}$,
I.~Boiarska$^{3}$,
K.~Bondarenko$^{27,57}$,
W.M.~Bonivento$^{14}$,
J.~Borburgh$^{44}$,
A.~Boyarsky$^{27,55}$,
R.~Brenner$^{43}$,
D.~Breton$^{4}$,
A. Brignoli$^{6}$,
V.~B\"{u}scher$^{10}$,
A.~Buonaura$^{47}$,
S.~Buontempo$^{15}$,
S.~Cadeddu$^{14}$,
M.~Calviani$^{44}$,
M.~Campanelli$^{53}$,
M.~Casolino$^{44}$,
N.~Charitonidis$^{44}$,
P.~Chau$^{10}$,
J.~Chauveau$^{5}$,
A.~Chepurnov$^{39}$,
M.~Chernyavskiy$^{32}$,
K.-Y.~Choi$^{26}$,
A.~Chumakov$^{2}$,
V.~Cicero$^{13}$,
M.~Climescu$^{10}$,
A.~Conaboy$^{6}$,
L.~Congedo$^{12,a}$,
K.~Cornelis$^{44}$,
M.~Cristinziani$^{11}$,
A.~Crupano$^{13}$,
G.M.~Dallavalle$^{13}$,
A.~Datwyler$^{47}$,
N.~D'Ambrosio$^{16}$,
G.~D'Appollonio$^{14,c}$,
R.~de~Asmundis$^{15}$,
J.~De~Carvalho~Saraiva$^{28}$,
G.~De~Lellis$^{15,34,44,d}$,
M.~de~Magistris$^{15,l}$,
A.~De~Roeck$^{44}$,
M.~De~Serio$^{12,a}$,
D.~De~Simone$^{47}$,
L.~Dedenko$^{39}$,
P.~Dergachev$^{34}$,
A.~Di~Crescenzo$^{15,44,d}$,
L.~Di~Giulio$^{44}$,
C.~Dib$^{2}$,
H.~Dijkstra$^{44}$,
V.~Dmitrenko$^{38}$,
L.A.~Dougherty$^{44}$,
A.~Dolmatov$^{33}$,
S.~Donskov$^{35}$,
V.~Drohan$^{55}$,
A.~Dubreuil$^{45}$,
O.~Durhan$^{48}$,
M.~Ehlert$^{6}$,
E.~Elikkaya$^{48}$,
T.~Enik$^{29}$,
A.~Etenko$^{33,38}$,
F.~Fabbri$^{13}$,
O.~Fedin$^{36}$,
F.~Fedotovs$^{52}$,
M.~Ferrillo$^{47}$,
M.~Ferro-Luzzi$^{44}$,
K.~Filippov$^{38}$,
R.A.~Fini$^{12}$,
H.~Fischer$^{7}$,
P.~Fonte$^{28}$,
C.~Franco$^{28}$,
M.~Fraser$^{44}$,
R.~Fresa$^{15,i,h}$,
R.~Froeschl$^{44}$,
T.~Fukuda$^{19}$,
G.~Galati$^{12,a}$,
J.~Gall$^{44}$,
L.~Gatignon$^{44}$,
G.~Gavrilov$^{36}$,
V.~Gentile$^{15,34,d}$,
B.~Goddard$^{44}$,
L.~Golinka-Bezshyyko$^{55}$,
A.~Golovatiuk$^{15,d}$,
V.~Golovtsov$^{36}$,
D.~Golubkov$^{30}$,
A.~Golutvin$^{52,34}$,
P.~Gorbounov$^{44}$,
D.~Gorbunov$^{31}$,
S.~Gorbunov$^{32}$,
V.~Gorkavenko$^{55}$,
M.~Gorshenkov$^{34}$,
V.~Grachev$^{38}$,
A.L.~Grandchamp$^{46}$,
E.~Graverini$^{46}$,
J.-L.~Grenard$^{44}$,
D.~Grenier$^{44}$,
V.~Grichine$^{32}$,
N.~Gruzinskii$^{36}$,
A.~M.~Guler$^{48}$,
Yu.~Guz$^{35}$,
G.J.~Haefeli$^{46}$,
C.~Hagner$^{8}$,
H.~Hakobyan$^{2}$,
I.W.~Harris$^{46}$,
E.~van~Herwijnen$^{44}$,
C.~Hessler$^{44}$,
A.~Hollnagel$^{10}$,
B.~Hosseini$^{52}$,
M.~Hushchyn$^{40}$,
G.~Iaselli$^{12,a}$,
A.~Iuliano$^{15,d}$,
R.~Jacobsson$^{44}$,
D.~Jokovi\'{c}$^{41}$,
M.~Jonker$^{44}$,
I.~Kadenko$^{55}$,
V.~Kain$^{44}$,
B.~Kaiser$^{8}$,
C.~Kamiscioglu$^{49}$,
D.~Karpenkov$^{34}$,
K.~Kershaw$^{44}$,
M.~Khabibullin$^{31}$,
E.~Khalikov$^{39}$,
G.~Khaustov$^{35}$,
G.~Khoriauli$^{10}$,
A.~Khotyantsev$^{31}$,
Y.G.~Kim$^{23}$,
V.~Kim$^{36,37}$,
N.~Kitagawa$^{19}$,
J.-W.~Ko$^{22}$,
K.~Kodama$^{17}$,
A.~Kolesnikov$^{29}$,
D.I.~Kolev$^{1}$,
V.~Kolosov$^{35}$,
M.~Komatsu$^{19}$,
A.~Kono$^{21}$,
N.~Konovalova$^{32,34}$,
S.~Kormannshaus$^{10}$,
I.~Korol$^{6}$,
I.~Korol'ko$^{30}$,
A.~Korzenev$^{45}$,
V.~Kostyukhin$^{11}$,
E.~Koukovini~Platia$^{44}$,
S.~Kovalenko$^{2}$,
I.~Krasilnikova$^{34}$,
Y.~Kudenko$^{31,38,g}$,
E.~Kurbatov$^{40}$,
P.~Kurbatov$^{34}$,
V.~Kurochka$^{31}$,
E.~Kuznetsova$^{36}$,
H.M.~Lacker$^{6}$,
M.~Lamont$^{44}$,
O.~Lantwin$^{47,34}$,
A.~Lauria$^{15,d}$,
K.S.~Lee$^{25}$,
K.Y.~Lee$^{22}$,
N.~Leonardo$^{28}$,
J.-M.~L\'{e}vy$^{5}$,
V.P.~Loschiavo$^{15,h}$,
L.~Lopes$^{28}$,
E.~Lopez~Sola$^{44}$,
F.~Lyons$^{7}$,
V.~Lyubovitskij$^{2}$,
J.~Maalmi$^{4}$,
A.-M.~Magnan$^{52}$,
V.~Maleev$^{36}$,
A.~Malinin$^{33}$,
Y.~Manabe$^{19}$,
A.K.~Managadze$^{39}$,
M.~Manfredi$^{44}$,
S.~Marsh$^{44}$,
A.M.~Marshall$^{50}$,
A.~Mefodev$^{31}$,
P.~Mermod$^{45}$,
A.~Miano$^{15,d}$,
S.~Mikado$^{20}$,
Yu.~Mikhaylov$^{35}$,
A.~Mikulenko$^{27}$,
D.A.~Milstead$^{42}$,
O.~Mineev$^{31}$,
A.~Montanari$^{13}$,
M.C.~Montesi$^{15,d}$,
K.~Morishima$^{19}$,
S.~Movchan$^{29}$,
Y.~Muttoni$^{44}$,
N.~Naganawa$^{19}$,
M.~Nakamura$^{19}$,
T.~Nakano$^{19}$,
S.~Nasybulin$^{36}$,
P.~Ninin$^{44}$,
A.~Nishio$^{19}$,
B.~Obinyakov$^{33}$,
S.~Ogawa$^{21}$,
N.~Okateva$^{32,34}$,
J.~Osborne$^{44}$,
M.~Ovchynnikov$^{27,55}$,
N.~Owtscharenko$^{11}$,
P.H.~Owen$^{47}$,
P.~Pacholek$^{44}$,
B.D.~Park$^{22}$,
A.~Pastore$^{12}$,
M.~Patel$^{52,34}$,
D.~Pereyma$^{30}$,
A.~Perillo-Marcone$^{44}$,
G.L.~Petkov$^{1}$,
K.~Petridis$^{50}$,
A.~Petrov$^{33}$,
D.~Podgrudkov$^{39}$,
V.~Poliakov$^{35}$,
N.~Polukhina$^{32,34,38}$,
J.~Prieto~Prieto$^{44}$,
M.~Prokudin$^{30}$,
A.~Prota$^{15,d}$,
A.~Quercia$^{15,d}$,
A.~Rademakers$^{44}$,
A.~Rakai$^{44}$,
F.~Ratnikov$^{40}$,
T.~Rawlings$^{51}$,
F.~Redi$^{46}$,
A.~Reghunath$^{6}$,
S.~Ricciardi$^{51}$,
M.~Rinaldesi$^{44}$,
Volodymyr~Rodin$^{55}$,
Viktor~Rodin$^{55}$,
P.~Robbe$^{4}$,
A.B.~Rodrigues~Cavalcante$^{46}$,
T.~Roganova$^{39}$,
H.~Rokujo$^{19}$,
G.~Rosa$^{15,d}$,
T.~Rovelli$^{13,b}$,
O.~Ruchayskiy$^{3}$,
T.~Ruf$^{44}$,
V.~Samoylenko$^{35}$,
V.~Samsonov$^{38}$,
F.~Sanchez~Galan$^{44}$,
P.~Santos~Diaz$^{44}$,
A.~Sanz~Ull$^{44}$,
O.~Sato$^{19}$,
E.S.~Savchenko$^{34}$,
J.S.~Schliwinski$^{6}$,
W.~Schmidt-Parzefall$^{8}$,
M.~Schumann$^{7}$,
N.~Serra$^{47}$,
S.~Sgobba$^{44}$,
O.~Shadura$^{55}$,
A.~Shakin$^{34}$,
M.~Shaposhnikov$^{46}$,
P.~Shatalov$^{31,34}$,
T.~Shchedrina$^{32,34}$,
L.~Shchutska$^{46}$,
V.~Shevchenko$^{32,34}$,
H.~Shibuya$^{21}$,
L.~Shihora$^{6}$,
S.~Shirobokov$^{52}$,
A.~Shustov$^{38}$,
S.B.~Silverstein$^{42}$,
S.~Simone$^{12,a}$,
R.~Simoniello$^{10}$,
M.~Skorokhvatov$^{38,33}$,
S.~Smirnov$^{38}$,
G.~Soares$^{28}$, 
J.Y.~Sohn$^{22}$,
A.~Sokolenko$^{55}$,
E.~Solodko$^{44}$,
N.~Starkov$^{33,34}$,
L.~Stoel$^{44}$,
M.E.~Stramaglia$^{46}$,
D.~Sukhonos$^{44}$,
Y.~Suzuki$^{19}$,
S.~Takahashi$^{18}$,
J.L.~Tastet$^{3}$,
P.~Teterin$^{38}$,
S.~Than~Naing$^{32}$,
I.~Timiryasov$^{46}$,
V.~Tioukov$^{15}$,
D.~Tommasini$^{44}$,
M.~Torii$^{19}$,
N.~Tosi$^{13}$,
D.~Treille$^{44}$,
R.~Tsenov$^{1,29}$,
S.~Ulin$^{38}$,
E.~Ursov$^{39}$,
A.~Ustyuzhanin$^{40,34}$,
Z.~Uteshev$^{38}$,
L.~Uvarov$^{36}$,
G.~Vankova-Kirilova$^{1}$,
F.~Vannucci$^{5}$,
P.~Venkova$^{6}$,
V.~Venturi$^{44}$,
I.~Vidulin$^{39}$,
S.~Vilchinski$^{55}$,
Heinz~Vincke$^{44}$,
Helmut~Vincke$^{44}$,
C.~Visone$^{15,d}$,
K.~Vlasik$^{38}$,
A.~Volkov$^{32,33}$,
R.~Voronkov$^{32}$,
S.~van~Waasen$^{9}$,
R.~Wanke$^{10}$,
P.~Wertelaers$^{44}$,
O.~Williams$^{44}$,
J.-K.~Woo$^{24}$,
M.~Wurm$^{10}$,
S.~Xella$^{3}$,
D.~Yilmaz$^{49}$,
A.U.~Yilmazer$^{49}$,
C.S.~Yoon$^{22}$,
Yu.~Zaytsev$^{30}$,
A.~Zelenov$^{36}$,
J.~Zimmerman$^{6}$


\vspace*{1cm}


{\footnotesize \it

$^{1}$Faculty of Physics, Sofia University, Sofia, Bulgaria\\
$^{2}$Universidad T\'ecnica Federico Santa Mar\'ia and Centro Cient\'ifico Tecnol\'ogico de Valpara\'iso, Valpara\'iso, Chile\\
$^{3}$Niels Bohr Institute, University of Copenhagen, Copenhagen, Denmark\\
$^{4}$LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit\'{e} Paris-Saclay, Orsay, France\\
$^{5}$LPNHE, IN2P3/CNRS, Sorbonne Universit\'{e}, Universit\'{e} Paris Diderot,F-75151 Paris, France\\
$^{6}$Humboldt-Universit\"{a}t zu Berlin, Berlin, Germany\\
$^{7}$Physikalisches Institut, Universit\"{a}t Freiburg, Freiburg, Germany\\
$^{8}$Universit\"{a}t Hamburg, Hamburg, Germany\\
$^{9}$Forschungszentrum J\"{u}lich GmbH (KFA),  J\"{u}lich , Germany\\
$^{10}$Institut f\"{u}r Physik and PRISMA Cluster of Excellence, Johannes Gutenberg Universit\"{a}t Mainz, Mainz, Germany\\
$^{11}$Universit\"{a}t Siegen, Siegen, Germany\\
$^{12}$Sezione INFN di Bari, Bari, Italy\\
$^{13}$Sezione INFN di Bologna, Bologna, Italy\\
$^{14}$Sezione INFN di Cagliari, Cagliari, Italy\\
$^{15}$Sezione INFN di Napoli, Napoli, Italy\\
$^{16}$Laboratori Nazionali dell'INFN di Gran Sasso, L'Aquila, Italy\\
$^{17}$Aichi University of Education, Kariya, Japan\\
$^{18}$Kobe University, Kobe, Japan\\
$^{19}$Nagoya University, Nagoya, Japan\\
$^{20}$College of Industrial Technology, Nihon University, Narashino, Japan\\
$^{21}$Toho University, Funabashi, Chiba, Japan\\
$^{22}$Physics Education Department \& RINS, Gyeongsang National University, Jinju, Korea\\
$^{23}$Gwangju National University of Education~$^{e}$, Gwangju, Korea\\
$^{24}$Jeju National University~$^{e}$, Jeju, Korea\\
$^{25}$Korea University, Seoul, Korea\\
$^{26}$Sungkyunkwan University~$^{e}$, Suwon-si, Gyeong Gi-do, Korea\\
$^{27}$University of Leiden, Leiden, The Netherlands\\
$^{28}$LIP, Laboratory of Instrumentation and Experimental Particle Physics, Portugal\\
^{29}$Joint Institute for Nuclear Research (JINR), Dubna, Russia\\
$^{30}$Institute of Theoretical and Experimental Physics (ITEP) NRC ``Kurchatov Institute``, Moscow, Russia\\
$^{31}$Institute for Nuclear Research of the Russian Academy of Sciences (INR RAS), Moscow, Russia\\
$^{32}$P.N.~Lebedev Physical Institute (LPI RAS), Moscow, Russia\\
$^{33}$National Research Centre ``Kurchatov Institute``, Moscow, Russia\\
$^{34}$National University of Science and Technology ``MISiS``, Moscow, Russia\\
$^{35}$Institute for High Energy Physics (IHEP) NRC ``Kurchatov Institute``, Protvino, Russia\\
$^{36}$Petersburg Nuclear Physics Institute (PNPI) NRC ``Kurchatov Institute``, Gatchina, Russia\\
$^{37}$St. Petersburg Polytechnic University (SPbPU)~$^{f}$, St. Petersburg, Russia\\
$^{38}$National Research Nuclear University (MEPhI), Moscow, Russia\\
$^{39}$Skobeltsyn Institute of Nuclear Physics of Moscow State University (SINP MSU), Moscow, Russia\\
$^{40}$Yandex School of Data Analysis, Moscow, Russia\\
$^{41}$Institute of Physics, University of Belgrade, Serbia\\
$^{42}$Stockholm University, Stockholm, Sweden\\
$^{43}$Uppsala University, Uppsala, Sweden\\
$^{44}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$^{45}$University of Geneva, Geneva, Switzerland\\
$^{46}$\'{E}cole Polytechnique F\'{e}d\'{e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$^{47}$Physik-Institut, Universit\"{a}t Z\"{u}rich, Z\"{u}rich, Switzerland\\
$^{48}$Middle East Technical University (METU), Ankara, Turkey\\
$^{49}$Ankara University, Ankara, Turkey\\
$^{50}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom \\
$^{51}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{52}$Imperial College London, London, United Kingdom\\
$^{53}$University College London, London, United Kingdom\\
$^{54}$University of Warwick, Warwick, United Kingdom\\
$^{55}$Taras Shevchenko National University of Kyiv, Kyiv, Ukraine\\
$^{a}$Universit\`{a} di Bari, Bari, Italy\\
$^{b}$Universit\`{a} di Bologna, Bologna, Italy\\
$^{c}$Universit\`{a} di Cagliari, Cagliari, Italy\\
$^{d}$Universit\`{a} di Napoli ``Federico II``, Napoli, Italy\\
$^{e}$Associated to Gyeongsang National University, Jinju, Korea\\
$^{f}$Associated to Petersburg Nuclear Physics Institute (PNPI), Gatchina, Russia\\
$^{g}$Also at Moscow Institute of Physics and Technology (MIPT),  Moscow Region, Russia\\
$^{h}$Consorzio CREATE, Napoli, Italy\\
$^{i}$Universit\`{a} della Basilicata, Potenza, Italy\\
$^{l}$Universit\`{a} di Napoli Parthenope, Napoli, Italy\\
}

Following the resolution of the CERN Council, Russian groups participating in the
SHiP project are not included in the author list of this document. We acknowledge the
contribution of the Russian scientists, in particular 

% \end{flushleft}




% \end{document}

==> lhcb-symbols-def.tex <==
%%% $Id: lhcb-symbols-def.tex 78711 2015-08-06 07:54:32Z apuignav $
%%% ======================================================================
%%% Purpose: Standard LHCb aliases
%%% Author: Originally Ulrik Egede, adapted by Tomasz Skwarnicki for templates,
%%% rewritten by Chris Parkes
%%% Maintainer : Ulrik Egede (2010 - 2012)
%%% Maintainer : Rolf Oldeman (2012 - 2014)
%%% =======================================================================

%%% To use this file outside the normal LHCb document environment, the
%%% following should be added in a preamble (before \begin{document}
%%%
%%%\usepackage{ifthen} 
%%%\newboolean{uprightparticles}
%%%\setboolean{uprightparticles}{false} %Set true for upright particle symbols
\usepackage{xspace} 
\usepackage{upgreek}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% The following is to ensure that the template automatically can process
%%% this file.
%%%
%%% Add comments with at least three %%% preceding.
%%% Add new sections with one % preceding
%%% Add new subsections with two %% preceding
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%
% Experiments
%%%%%%%%%%%%%
\def\lhcb {\mbox{LHCb}\xspace}
\def\atlas  {\mbox{ATLAS}\xspace}
\def\cms    {\mbox{CMS}\xspace}
\def\alice  {\mbox{ALICE}\xspace}
\def\babar  {\mbox{BaBar}\xspace}
\def\belle  {\mbox{Belle}\xspace}
\def\cleo   {\mbox{CLEO}\xspace}
\def\cdf    {\mbox{CDF}\xspace}
\def\dzero  {\mbox{D0}\xspace}
\def\aleph  {\mbox{ALEPH}\xspace}
\def\delphi {\mbox{DELPHI}\xspace}
\def\opal   {\mbox{OPAL}\xspace}
\def\lthree {\mbox{L3}\xspace}
\def\sld    {\mbox{SLD}\xspace}
%%%\def\argus  {\mbox{ARGUS}\xspace}
%%%\def\uaone  {\mbox{UA1}\xspace}
%%%\def\uatwo  {\mbox{UA2}\xspace}
%%%\def\ux85 {\mbox{UX85}\xspace}
\def\cern {\mbox{CERN}\xspace}
\def\lhc    {\mbox{LHC}\xspace}
\def\lep    {\mbox{LEP}\xspace}
\def\tevatron {Tevatron\xspace}

%% LHCb sub-detectors and sub-systems

%%%\def\pu     {PU\xspace}
\def\velo   {VELO\xspace}
\def\rich   {RICH\xspace}
\def\richone {RICH1\xspace}
\def\richtwo {RICH2\xspace}
\def\ttracker {TT\xspace}
\def\intr   {IT\xspace}
\def\st     {ST\xspace}
\def\ot     {OT\xspace}
%%%\def\Tone   {T1\xspace}
%%%\def\Ttwo   {T2\xspace}
%%%\def\Tthree {T3\xspace}
%%%\def\Mone   {M1\xspace}
%%%\def\Mtwo   {M2\xspace}
%%%\def\Mthree {M3\xspace}
%%%\def\Mfour  {M4\xspace}
%%%\def\Mfive  {M5\xspace}
\def\spd    {SPD\xspace}
\def\presh  {PS\xspace}
\def\ecal   {ECAL\xspace}
\def\hcal   {HCAL\xspace}
%%%\def\bcm    {BCM\xspace}
\def\MagUp {\mbox{\em Mag\kern -0.05em Up}\xspace}
\def\MagDown {\mbox{\em MagDown}\xspace}

\def\ode    {ODE\xspace}
\def\daq    {DAQ\xspace}
\def\tfc    {TFC\xspace}
\def\ecs    {ECS\xspace}
\def\lone   {L0\xspace}
\def\hlt    {HLT\xspace}
\def\hltone {HLT1\xspace}
\def\hlttwo {HLT2\xspace}

%%% Upright (not slanted) Particles

\ifthenelse{\boolean{uprightparticles}}%
{\def\Palpha      {\ensuremath{\upalpha}\xspace}
 \def\Pbeta       {\ensuremath{\upbeta}\xspace}
 \def\Pgamma      {\ensuremath{\upgamma}\xspace}                 
 \def\Pdelta      {\ensuremath{\updelta}\xspace}                 
 \def\Pepsilon    {\ensuremath{\upepsilon}\xspace}                 
 \def\Pvarepsilon {\ensuremath{\upvarepsilon}\xspace}                 
 \def\Pzeta       {\ensuremath{\upzeta}\xspace}                 
 \def\Peta        {\ensuremath{\upeta}\xspace}                 
 \def\Ptheta      {\ensuremath{\uptheta}\xspace}                 
 \def\Pvartheta   {\ensuremath{\upvartheta}\xspace}                 
 \def\Piota       {\ensuremath{\upiota}\xspace}                 
 \def\Pkappa      {\ensuremath{\upkappa}\xspace}                 
 \def\Plambda     {\ensuremath{\uplambda}\xspace}                 
 \def\Pmu         {\ensuremath{\upmu}\xspace}                 
 \def\Pnu         {\ensuremath{\upnu}\xspace}                 
 \def\Pxi         {\ensuremath{\upxi}\xspace}                 
 \def\Ppi         {\ensuremath{\uppi}\xspace}                 
 \def\Pvarpi      {\ensuremath{\upvarpi}\xspace}                 
 \def\Prho        {\ensuremath{\uprho}\xspace}                 
 \def\Pvarrho     {\ensuremath{\upvarrho}\xspace}                 
 \def\Ptau        {\ensuremath{\uptau}\xspace}                 
 \def\Pupsilon    {\ensuremath{\upupsilon}\xspace}                 
 \def\Pphi        {\ensuremath{\upphi}\xspace}                 
 \def\Pvarphi     {\ensuremath{\upvarphi}\xspace}                 
 \def\Pchi        {\ensuremath{\upchi}\xspace}                 
 \def\Ppsi        {\ensuremath{\uppsi}\xspace}                 
 \def\Pomega      {\ensuremath{\upomega}\xspace}                 

 \def\PDelta      {\ensuremath{\Delta}\xspace}                 
 \def\PXi      {\ensuremath{\Xi}\xspace}                 
 \def\PLambda      {\ensuremath{\Lambda}\xspace}                 
 \def\PSigma      {\ensuremath{\Sigma}\xspace}                 
 \def\POmega      {\ensuremath{\Omega}\xspace}                 
 \def\PUpsilon      {\ensuremath{\Upsilon}\xspace}                 
 
 %\mathchardef\Deltares="7101
 %\mathchardef\Xi="7104
 %\mathchardef\Lambda="7103
 %\mathchardef\Sigma="7106
 %\mathchardef\Omega="710A


 \def\PA      {\ensuremath{\mathrm{A}}\xspace}                 
 \def\PB      {\ensuremath{\mathrm{B}}\xspace}                 
 \def\PC      {\ensuremath{\mathrm{C}}\xspace}                 
 \def\PD      {\ensuremath{\mathrm{D}}\xspace}                 
 \def\PE      {\ensuremath{\mathrm{E}}\xspace}                 
 \def\PF      {\ensuremath{\mathrm{F}}\xspace}                 
 \def\PG      {\ensuremath{\mathrm{G}}\xspace}                 
 \def\PH      {\ensuremath{\mathrm{H}}\xspace}                 
 \def\PI      {\ensuremath{\mathrm{I}}\xspace}                 
 \def\PJ      {\ensuremath{\mathrm{J}}\xspace}                 
 \def\PK      {\ensuremath{\mathrm{K}}\xspace}                 
 \def\PL      {\ensuremath{\mathrm{L}}\xspace}                 
 \def\PM      {\ensuremath{\mathrm{M}}\xspace}                 
 \def\PN      {\ensuremath{\mathrm{N}}\xspace}                 
 \def\PO      {\ensuremath{\mathrm{O}}\xspace}                 
 \def\PP      {\ensuremath{\mathrm{P}}\xspace}                 
 \def\PQ      {\ensuremath{\mathrm{Q}}\xspace}                 
 \def\PR      {\ensuremath{\mathrm{R}}\xspace}                 
 \def\PS      {\ensuremath{\mathrm{S}}\xspace}                 
 \def\PT      {\ensuremath{\mathrm{T}}\xspace}                 
 \def\PU      {\ensuremath{\mathrm{U}}\xspace}                 
 \def\PV      {\ensuremath{\mathrm{V}}\xspace}                 
 \def\PW      {\ensuremath{\mathrm{W}}\xspace}                 
 \def\PX      {\ensuremath{\mathrm{X}}\xspace}                 
 \def\PY      {\ensuremath{\mathrm{Y}}\xspace}                 
 \def\PZ      {\ensuremath{\mathrm{Z}}\xspace}                 
 \def\Pa      {\ensuremath{\mathrm{a}}\xspace}                 
 \def\Pb      {\ensuremath{\mathrm{b}}\xspace}                 
 \def\Pc      {\ensuremath{\mathrm{c}}\xspace}                 
 \def\Pd      {\ensuremath{\mathrm{d}}\xspace}                 
 \def\Pe      {\ensuremath{\mathrm{e}}\xspace}                 
 \def\Pf      {\ensuremath{\mathrm{f}}\xspace}                 
 \def\Pg      {\ensuremath{\mathrm{g}}\xspace}                 
 \def\Ph      {\ensuremath{\mathrm{h}}\xspace}                 
 \def\Pi      {\ensuremath{\mathrm{i}}\xspace}                 
 \def\Pj      {\ensuremath{\mathrm{j}}\xspace}                 
 \def\Pk      {\ensuremath{\mathrm{k}}\xspace}                 
 \def\Pl      {\ensuremath{\mathrm{l}}\xspace}                 
 \def\Pm      {\ensuremath{\mathrm{m}}\xspace}                 
 \def\Pn      {\ensuremath{\mathrm{n}}\xspace}                 
 \def\Po      {\ensuremath{\mathrm{o}}\xspace}                 
 \def\Pp      {\ensuremath{\mathrm{p}}\xspace}                 
 \def\Pq      {\ensuremath{\mathrm{q}}\xspace}                 
 \def\Pr      {\ensuremath{\mathrm{r}}\xspace}                 
 \def\Ps      {\ensuremath{\mathrm{s}}\xspace}                 
 \def\Pt      {\ensuremath{\mathrm{t}}\xspace}                 
 \def\Pu      {\ensuremath{\mathrm{u}}\xspace}                 
 \def\Pv      {\ensuremath{\mathrm{v}}\xspace}                 
 \def\Pw      {\ensuremath{\mathrm{w}}\xspace}                 
 \def\Px      {\ensuremath{\mathrm{x}}\xspace}                 
 \def\Py      {\ensuremath{\mathrm{y}}\xspace}                 
 \def\Pz      {\ensuremath{\mathrm{z}}\xspace}                 
}
{\def\Palpha      {\ensuremath{\alpha}\xspace}
 \def\Pbeta       {\ensuremath{\beta}\xspace}
 \def\Pgamma      {\ensuremath{\gamma}\xspace}                 
 \def\Pdelta      {\ensuremath{\delta}\xspace}                 
 \def\Pepsilon    {\ensuremath{\epsilon}\xspace}                 
 \def\Pvarepsilon {\ensuremath{\varepsilon}\xspace}                 
 \def\Pzeta       {\ensuremath{\zeta}\xspace}                 
 \def\Peta        {\ensuremath{\eta}\xspace}                 
 \def\Ptheta      {\ensuremath{\theta}\xspace}                 
 \def\Pvartheta   {\ensuremath{\vartheta}\xspace}                 
 \def\Piota       {\ensuremath{\iota}\xspace}                 
 \def\Pkappa      {\ensuremath{\kappa}\xspace}                 
 \def\Plambda     {\ensuremath{\lambda}\xspace}                 
 \def\Pmu         {\ensuremath{\mu}\xspace}                 
 \def\Pnu         {\ensuremath{\nu}\xspace}                 
 \def\Pxi         {\ensuremath{\xi}\xspace}                 
 \def\Ppi         {\ensuremath{\pi}\xspace}                 
 \def\Pvarpi      {\ensuremath{\varpi}\xspace}                 
 \def\Prho        {\ensuremath{\rho}\xspace}                 
 \def\Pvarrho     {\ensuremath{\varrho}\xspace}                 
 \def\Ptau        {\ensuremath{\tau}\xspace}                 
 \def\Pupsilon    {\ensuremath{\upsilon}\xspace}                 
 \def\Pphi        {\ensuremath{\phi}\xspace}                 
 \def\Pvarphi     {\ensuremath{\varphi}\xspace}                 
 \def\Pchi        {\ensuremath{\chi}\xspace}                 
 \def\Ppsi        {\ensuremath{\psi}\xspace}                 
 \def\Pomega      {\ensuremath{\omega}\xspace}                 
 \mathchardef\PDelta="7101
 \mathchardef\PXi="7104
 \mathchardef\PLambda="7103
 \mathchardef\PSigma="7106
 \mathchardef\POmega="710A
 \mathchardef\PUpsilon="7107
 \def\PA      {\ensuremath{A}\xspace}                 
 \def\PB      {\ensuremath{B}\xspace}                 
 \def\PC      {\ensuremath{C}\xspace}                 
 \def\PD      {\ensuremath{D}\xspace}                 
 \def\PE      {\ensuremath{E}\xspace}                 
 \def\PF      {\ensuremath{F}\xspace}                 
 \def\PG      {\ensuremath{G}\xspace}                 
 \def\PH      {\ensuremath{H}\xspace}                 
 \def\PI      {\ensuremath{I}\xspace}                 
 \def\PJ      {\ensuremath{J}\xspace}                 
 \def\PK      {\ensuremath{K}\xspace}                 
 \def\PL      {\ensuremath{L}\xspace}                 
 \def\PM      {\ensuremath{M}\xspace}                 
 \def\PN      {\ensuremath{N}\xspace}                 
 \def\PO      {\ensuremath{O}\xspace}                 
 \def\PP      {\ensuremath{P}\xspace}                 
 \def\PQ      {\ensuremath{Q}\xspace}                 
 \def\PR      {\ensuremath{R}\xspace}                 
 \def\PS      {\ensuremath{S}\xspace}                 
 \def\PT      {\ensuremath{T}\xspace}                 
 \def\PU      {\ensuremath{U}\xspace}                 
 \def\PV      {\ensuremath{V}\xspace}                 
 \def\PW      {\ensuremath{W}\xspace}                 
 \def\PX      {\ensuremath{X}\xspace}                 
 \def\PY      {\ensuremath{Y}\xspace}                 
 \def\PZ      {\ensuremath{Z}\xspace}                 
 \def\Pa      {\ensuremath{a}\xspace}                 
 \def\Pb      {\ensuremath{b}\xspace}                 
 \def\Pc      {\ensuremath{c}\xspace}                 
 \def\Pd      {\ensuremath{d}\xspace}                 
 \def\Pe      {\ensuremath{e}\xspace}                 
 \def\Pf      {\ensuremath{f}\xspace}                 
 \def\Pg      {\ensuremath{g}\xspace}                 
 \def\Ph      {\ensuremath{h}\xspace}                 
 \def\Pi      {\ensuremath{i}\xspace}                 
 \def\Pj      {\ensuremath{j}\xspace}                 
 \def\Pk      {\ensuremath{k}\xspace}                 
 \def\Pl      {\ensuremath{l}\xspace}                 
 \def\Pm      {\ensuremath{m}\xspace}                 
 \def\Pn      {\ensuremath{n}\xspace}                 
 \def\Po      {\ensuremath{o}\xspace}                 
 \def\Pp      {\ensuremath{p}\xspace}                 
 \def\Pq      {\ensuremath{q}\xspace}                 
 \def\Pr      {\ensuremath{r}\xspace}                 
 \def\Ps      {\ensuremath{s}\xspace}                 
 \def\Pt      {\ensuremath{t}\xspace}                 
 \def\Pu      {\ensuremath{u}\xspace}                 
 \def\Pv      {\ensuremath{v}\xspace}                 
 \def\Pw      {\ensuremath{w}\xspace}                 
 \def\Px      {\ensuremath{x}\xspace}                 
 \def\Py      {\ensuremath{y}\xspace}                 
 \def\Pz      {\ensuremath{z}\xspace}                 
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Particles
\makeatletter
\ifcase \@ptsize \relax% 10pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{4}{5}}% \tiny: 5/6
\or% 11pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{5}{6}}% \tiny: 6/7
\or% 12pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{5}{6}}% \tiny: 6/7
\fi
\makeatother


\DeclareRobustCommand{\optbar}[1]{\shortstack{{\miniscule (\rule[.5ex]{1.25em}{.18mm})}
  \\ [-.7ex] $#1$}}


%% Leptons

\let\emi\en
\def\electron   {{\ensuremath{\Pe}}\xspace}
\def\en         {{\ensuremath{\Pe^-}}\xspace}   % electron negative (\em is taken)
\def\ep         {{\ensuremath{\Pe^+}}\xspace}
\def\epm        {{\ensuremath{\Pe^\pm}}\xspace} 
\def\epem       {{\ensuremath{\Pe^+\Pe^-}}\xspace}
%%%\def\ee         {\ensuremath{\Pe^-\Pe^-}\xspace}

\def\muon       {{\ensuremath{\Pmu}}\xspace}
\def\mup        {{\ensuremath{\Pmu^+}}\xspace}
\def\mun        {{\ensuremath{\Pmu^-}}\xspace} % muon negative (\mum is taken)
\def\mumu       {{\ensuremath{\Pmu^+\Pmu^-}}\xspace}

\def\tauon      {{\ensuremath{\Ptau}}\xspace}
\def\taup       {{\ensuremath{\Ptau^+}}\xspace}
\def\taum       {{\ensuremath{\Ptau^-}}\xspace}
\def\tautau     {{\ensuremath{\Ptau^+\Ptau^-}}\xspace}

\def\lepton     {{\ensuremath{\ell}}\xspace}
\def\ellm       {{\ensuremath{\ell^-}}\xspace}
\def\ellp       {{\ensuremath{\ell^+}}\xspace}
%%%\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\neu        {{\ensuremath{\Pnu}}\xspace}
\def\neub       {{\ensuremath{\overline{\Pnu}}}\xspace}
%%%\def\nuenueb    {\ensuremath{\neu\neub}\xspace}
\def\neue       {{\ensuremath{\neu_e}}\xspace}
\def\neueb      {{\ensuremath{\neub_e}}\xspace}
%%%\def\neueneueb  {\ensuremath{\neue\neueb}\xspace}
\def\neum       {{\ensuremath{\neu_\mu}}\xspace}
\def\neumb      {{\ensuremath{\neub_\mu}}\xspace}
%%%\def\neumneumb  {\ensuremath{\neum\neumb}\xspace}
\def\neut       {{\ensuremath{\neu_\tau}}\xspace}
\def\neutb      {{\ensuremath{\neub_\tau}}\xspace}
%%%\def\neutneutb  {\ensuremath{\neut\neutb}\xspace}
\def\neul       {{\ensuremath{\neu_\ell}}\xspace}
\def\neulb      {{\ensuremath{\neub_\ell}}\xspace}
%%%\def\neulneulb  {\ensuremath{\neul\neulb}\xspace}

%% Gauge bosons and scalars

\def\g      {{\ensuremath{\Pgamma}}\xspace}
\def\H      {{\ensuremath{\PH^0}}\xspace}
\def\Hp     {{\ensuremath{\PH^+}}\xspace}
\def\Hm     {{\ensuremath{\PH^-}}\xspace}
\def\Hpm    {{\ensuremath{\PH^\pm}}\xspace}
\def\W      {{\ensuremath{\PW}}\xspace}
\def\Wp     {{\ensuremath{\PW^+}}\xspace}
\def\Wm     {{\ensuremath{\PW^-}}\xspace}
\def\Wpm    {{\ensuremath{\PW^\pm}}\xspace}
\def\Z      {{\ensuremath{\PZ}}\xspace}

%% Quarks

\def\quark     {{\ensuremath{\Pq}}\xspace}
\def\quarkbar  {{\ensuremath{\overline \quark}}\xspace}
\def\qqbar     {{\ensuremath{\quark\quarkbar}}\xspace}
\def\uquark    {{\ensuremath{\Pu}}\xspace}
\def\uquarkbar {{\ensuremath{\overline \uquark}}\xspace}
\def\uubar     {{\ensuremath{\uquark\uquarkbar}}\xspace}
\def\dquark    {{\ensuremath{\Pd}}\xspace}
\def\dquarkbar {{\ensuremath{\overline \dquark}}\xspace}
\def\ddbar     {{\ensuremath{\dquark\dquarkbar}}\xspace}
\def\squark    {{\ensuremath{\Ps}}\xspace}
\def\squarkbar {{\ensuremath{\overline \squark}}\xspace}
\def\ssbar     {{\ensuremath{\squark\squarkbar}}\xspace}
\def\cquark    {{\ensuremath{\Pc}}\xspace}
\def\cquarkbar {{\ensuremath{\overline \cquark}}\xspace}
\def\ccbar     {{\ensuremath{\cquark\cquarkbar}}\xspace}
\def\bquark    {{\ensuremath{\Pb}}\xspace}
\def\bquarkbar {{\ensuremath{\overline \bquark}}\xspace}
\def\bbbar     {{\ensuremath{\bquark\bquarkbar}}\xspace}
\def\tquark    {{\ensuremath{\Pt}}\xspace}
\def\tquarkbar {{\ensuremath{\overline \tquark}}\xspace}
\def\ttbar     {{\ensuremath{\tquark\tquarkbar}}\xspace}

%% Light mesons

\def\hadron {{\ensuremath{\Ph}}\xspace}
\def\pion   {{\ensuremath{\Ppi}}\xspace}
\def\piz    {{\ensuremath{\pion^0}}\xspace}
\def\pizs   {{\ensuremath{\pion^0\mbox\,\mathrm{s}}}\xspace}
\def\pip    {{\ensuremath{\pion^+}}\xspace}
\def\pim    {{\ensuremath{\pion^-}}\xspace}
\def\pipm   {{\ensuremath{\pion^\pm}}\xspace}
\def\pimp   {{\ensuremath{\pion^\mp}}\xspace}

\def\rhomeson {{\ensuremath{\Prho}}\xspace}
\def\rhoz     {{\ensuremath{\rhomeson^0}}\xspace}
\def\rhop     {{\ensuremath{\rhomeson^+}}\xspace}
\def\rhom     {{\ensuremath{\rhomeson^-}}\xspace}
\def\rhopm    {{\ensuremath{\rhomeson^\pm}}\xspace}
\def\rhomp    {{\ensuremath{\rhomeson^\mp}}\xspace}

\def\kaon    {{\ensuremath{\PK}}\xspace}
%%% do NOT use ensuremath here
  \def\Kbar    {{\kern 0.2em\overline{\kern -0.2em \PK}{}}\xspace}
\def\Kb      {{\ensuremath{\Kbar}}\xspace}
\def\KorKbar    {\kern 0.18em\optbar{\kern -0.18em K}{}\xspace}
\def\Kz      {{\ensuremath{\kaon^0}}\xspace}
\def\Kzb     {{\ensuremath{\Kbar{}^0}}\xspace}
\def\Kp      {{\ensuremath{\kaon^+}}\xspace}
\def\Km      {{\ensuremath{\kaon^-}}\xspace}
\def\Kpm     {{\ensuremath{\kaon^\pm}}\xspace}
\def\Kmp     {{\ensuremath{\kaon^\mp}}\xspace}
\def\KS      {{\ensuremath{\kaon^0_{\mathrm{ \scriptscriptstyle S}}}}\xspace}
\def\KL      {{\ensuremath{\kaon^0_{\mathrm{ \scriptscriptstyle L}}}}\xspace}
\def\Kstarz  {{\ensuremath{\kaon^{*0}}}\xspace}
\def\Kstarzb {{\ensuremath{\Kbar{}^{*0}}}\xspace}
\def\Kstar   {{\ensuremath{\kaon^*}}\xspace}
\def\Kstarb  {{\ensuremath{\Kbar{}^*}}\xspace}
\def\Kstarp  {{\ensuremath{\kaon^{*+}}}\xspace}
\def\Kstarm  {{\ensuremath{\kaon^{*-}}}\xspace}
\def\Kstarpm {{\ensuremath{\kaon^{*\pm}}}\xspace}
\def\Kstarmp {{\ensuremath{\kaon^{*\mp}}}\xspace}

\newcommand{\etaz}{\ensuremath{\Peta}\xspace}
\newcommand{\etapr}{\ensuremath{\Peta^{\prime}}\xspace}
\newcommand{\phiz}{\ensuremath{\Pphi}\xspace}
\newcommand{\omegaz}{\ensuremath{\Pomega}\xspace}

%% Heavy mesons

%%% do NOT use ensuremath here
  \def\Dbar    {{\kern 0.2em\overline{\kern -0.2em \PD}{}}\xspace}
\def\D       {{\ensuremath{\PD}}\xspace}
\def\Db      {{\ensuremath{\Dbar}}\xspace}
\def\DorDbar    {\kern 0.18em\optbar{\kern -0.18em D}{}\xspace}
\def\Dz      {{\ensuremath{\D^0}}\xspace}
\def\Dzb     {{\ensuremath{\Dbar{}^0}}\xspace}
\def\Dp      {{\ensuremath{\D^+}}\xspace}
\def\Dm      {{\ensuremath{\D^-}}\xspace}
\def\Dpm     {{\ensuremath{\D^\pm}}\xspace}
\def\Dmp     {{\ensuremath{\D^\mp}}\xspace}
\def\Dstar   {{\ensuremath{\D^*}}\xspace}
\def\Dstarb  {{\ensuremath{\Dbar{}^*}}\xspace}
\def\Dstarz  {{\ensuremath{\D^{*0}}}\xspace}
\def\Dstarzb {{\ensuremath{\Dbar{}^{*0}}}\xspace}
\def\Dstarp  {{\ensuremath{\D^{*+}}}\xspace}
\def\Dstarm  {{\ensuremath{\D^{*-}}}\xspace}
\def\Dstarpm {{\ensuremath{\D^{*\pm}}}\xspace}
\def\Dstarmp {{\ensuremath{\D^{*\mp}}}\xspace}
\def\Ds      {{\ensuremath{\D^+_\squark}}\xspace}
\def\Dsp     {{\ensuremath{\D^+_\squark}}\xspace}
\def\Dsm     {{\ensuremath{\D^-_\squark}}\xspace}
\def\Dspm    {{\ensuremath{\D^{\pm}_\squark}}\xspace}
\def\Dsmp    {{\ensuremath{\D^{\mp}_\squark}}\xspace}
\def\Dss     {{\ensuremath{\D^{*+}_\squark}}\xspace}
\def\Dssp    {{\ensuremath{\D^{*+}_\squark}}\xspace}
\def\Dssm    {{\ensuremath{\D^{*-}_\squark}}\xspace}
\def\Dsspm   {{\ensuremath{\D^{*\pm}_\squark}}\xspace}
\def\Dssmp   {{\ensuremath{\D^{*\mp}_\squark}}\xspace}

\def\B       {{\ensuremath{\PB}}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {{\ensuremath{\kern 0.18em\overline{\kern -0.18em \PB}{}}}\xspace}
\def\Bb      {{\ensuremath{\Bbar}}\xspace}
\def\BorBbar    {\kern 0.18em\optbar{\kern -0.18em B}{}\xspace}
\def\Bz      {{\ensuremath{\B^0}}\xspace}
\def\Bzb     {{\ensuremath{\Bbar{}^0}}\xspace}
\def\Bu      {{\ensuremath{\B^+}}\xspace}
\def\Bub     {{\ensuremath{\B^-}}\xspace}
\def\Bp      {{\ensuremath{\Bu}}\xspace}
\def\Bm      {{\ensuremath{\Bub}}\xspace}
\def\Bpm     {{\ensuremath{\B^\pm}}\xspace}
\def\Bmp     {{\ensuremath{\B^\mp}}\xspace}
\def\Bd      {{\ensuremath{\B^0}}\xspace}
\def\Bs      {{\ensuremath{\B^0_\squark}}\xspace}
\def\Bsb     {{\ensuremath{\Bbar{}^0_\squark}}\xspace}
\def\Bdb     {{\ensuremath{\Bbar{}^0}}\xspace}
\def\Bc      {{\ensuremath{\B_\cquark^+}}\xspace}
\def\Bcp     {{\ensuremath{\B_\cquark^+}}\xspace}
\def\Bcm     {{\ensuremath{\B_\cquark^-}}\xspace}
\def\Bcpm    {{\ensuremath{\B_\cquark^\pm}}\xspace}

%% Onia

\def\jpsi     {{\ensuremath{{\PJ\mskip -3mu/\mskip -2mu\Ppsi\mskip 2mu}}}\xspace}
\def\psitwos  {{\ensuremath{\Ppsi{(2S)}}}\xspace}
\def\psiprpr  {{\ensuremath{\Ppsi(3770)}}\xspace}
\def\etac     {{\ensuremath{\Peta_\cquark}}\xspace}
\def\chiczero {{\ensuremath{\Pchi_{\cquark 0}}}\xspace}
\def\chicone  {{\ensuremath{\Pchi_{\cquark 1}}}\xspace}
\def\chictwo  {{\ensuremath{\Pchi_{\cquark 2}}}\xspace}
  %\mathchardef\Upsilon="7107
  \def\Y#1S{\ensuremath{\PUpsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {{\Y1S}}
\def\TwoS  {{\Y2S}}
\def\ThreeS{{\Y3S}}
\def\FourS {{\Y4S}}
\def\FiveS {{\Y5S}}

\def\chic  {{\ensuremath{\Pchi_{c}}}\xspace}

%% Baryons

\def\proton      {{\ensuremath{\Pp}}\xspace}
\def\antiproton  {{\ensuremath{\overline \proton}}\xspace}
\def\neutron     {{\ensuremath{\Pn}}\xspace}
\def\antineutron {{\ensuremath{\overline \neutron}}\xspace}
\def\Deltares    {{\ensuremath{\PDelta}}\xspace}
\def\Deltaresbar {{\ensuremath{\overline \Deltares}}\xspace}
\def\Xires       {{\ensuremath{\PXi}}\xspace}
\def\Xiresbar    {{\ensuremath{\overline \Xires}}\xspace}
\def\Lz          {{\ensuremath{\PLambda}}\xspace}
\def\Lbar        {{\ensuremath{\kern 0.1em\overline{\kern -0.1em\PLambda}}}\xspace}
\def\LorLbar    {\kern 0.18em\optbar{\kern -0.18em \PLambda}{}\xspace}
\def\Lambdares   {{\ensuremath{\PLambda}}\xspace}
\def\Lambdaresbar{{\ensuremath{\Lbar}}\xspace}
\def\Sigmares    {{\ensuremath{\PSigma}}\xspace}
\def\Sigmaresbar {{\ensuremath{\overline \Sigmares}}\xspace}
\def\Omegares    {{\ensuremath{\POmega}}\xspace}
\def\Omegaresbar {{\ensuremath{\overline \POmega}}\xspace}

%%% do NOT use ensuremath here
 % \def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
 % \def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
 % \def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
 % \def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
 % \def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
 % \def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\Lb      {{\ensuremath{\Lz^0_\bquark}}\xspace}
\def\Lbbar   {{\ensuremath{\Lbar{}^0_\bquark}}\xspace}
\def\Lc      {{\ensuremath{\Lz^+_\cquark}}\xspace}
\def\Lcbar   {{\ensuremath{\Lbar{}^-_\cquark}}\xspace}
\def\Xib     {{\ensuremath{\Xires_\bquark}}\xspace}
\def\Xibz    {{\ensuremath{\Xires^0_\bquark}}\xspace}
\def\Xibm    {{\ensuremath{\Xires^-_\bquark}}\xspace}
\def\Xibbar  {{\ensuremath{\Xiresbar{}_\bquark}}\xspace}
\def\Xibbarz {{\ensuremath{\Xiresbar{}_\bquark^0}}\xspace}
\def\Xibbarp {{\ensuremath{\Xiresbar{}_\bquark^+}}\xspace}
\def\Xic     {{\ensuremath{\Xires_\cquark}}\xspace}
\def\Xicz    {{\ensuremath{\Xires^0_\cquark}}\xspace}
\def\Xicp    {{\ensuremath{\Xires^+_\cquark}}\xspace}
\def\Xicbar  {{\ensuremath{\Xiresbar{}_\cquark}}\xspace}
\def\Xicbarz {{\ensuremath{\Xiresbar{}_\cquark^0}}\xspace}
\def\Xicbarm {{\ensuremath{\Xiresbar{}_\cquark^-}}\xspace}
\def\Omegac    {{\ensuremath{\Omegares^0_\cquark}}\xspace}
\def\Omegacbar {{\ensuremath{\Omegaresbar{}_\cquark^0}}\xspace}
\def\Omegab    {{\ensuremath{\Omegares^-_\bquark}}\xspace}
\def\Omegabbar {{\ensuremath{\Omegaresbar{}_\bquark^+}}\xspace}

%%%%%%%%%%%%%%%%%%
% Physics symbols
%%%%%%%%%%%%%%%%%

%% Decays
\def\BF         {{\ensuremath{\mathcal{B}}}\xspace}
\def\BRvis      {{\ensuremath{\BR_{\mathrm{{vis}}}}}}
\def\BR         {\BF}
\newcommand{\decay}[2]{\ensuremath{#1\!\to #2}\xspace}         % {\Pa}{\Pb \Pc}
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}

%% Lifetimes
\newcommand{\tauBs}{{\ensuremath{\tau_{\Bs}}}\xspace}
\newcommand{\tauBd}{{\ensuremath{\tau_{\Bd}}}\xspace}
\newcommand{\tauBz}{{\ensuremath{\tau_{\Bz}}}\xspace}
\newcommand{\tauBu}{{\ensuremath{\tau_{\Bp}}}\xspace}
\newcommand{\tauDp}{{\ensuremath{\tau_{\Dp}}}\xspace}
\newcommand{\tauDz}{{\ensuremath{\tau_{\Dz}}}\xspace}
\newcommand{\tauL}{{\ensuremath{\tau_{\mathrm{ L}}}}\xspace}
\newcommand{\tauH}{{\ensuremath{\tau_{\mathrm{ H}}}}\xspace}

%% Masses
\newcommand{\mBd}{{\ensuremath{m_{\Bd}}}\xspace}
\newcommand{\mBp}{{\ensuremath{m_{\Bp}}}\xspace}
\newcommand{\mBs}{{\ensuremath{m_{\Bs}}}\xspace}
\newcommand{\mBc}{{\ensuremath{m_{\Bc}}}\xspace}
\newcommand{\mLb}{{\ensuremath{m_{\Lb}}}\xspace}

%% EW theory, groups
\def\grpsuthree {{\ensuremath{\mathrm{SU}(3)}}\xspace}
\def\grpsutw    {{\ensuremath{\mathrm{SU}(2)}}\xspace}
\def\grpuone    {{\ensuremath{\mathrm{U}(1)}}\xspace}

\def\ssqtw   {{\ensuremath{\sin^{2}\!\theta_{\mathrm{W}}}}\xspace}
\def\csqtw   {{\ensuremath{\cos^{2}\!\theta_{\mathrm{W}}}}\xspace}
\def\stw     {{\ensuremath{\sin\theta_{\mathrm{W}}}}\xspace}
\def\ctw     {{\ensuremath{\cos\theta_{\mathrm{W}}}}\xspace}
\def\ssqtwef {{\ensuremath{{\sin}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\csqtwef {{\ensuremath{{\cos}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\stwef   {{\ensuremath{\sin\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\ctwef   {{\ensuremath{\cos\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\gv      {{\ensuremath{g_{\mbox{\tiny V}}}}\xspace}
\def\ga      {{\ensuremath{g_{\mbox{\tiny A}}}}\xspace}

\def\order   {{\ensuremath{\mathcal{O}}}\xspace}
\def\ordalph {{\ensuremath{\mathcal{O}(\alpha)}}\xspace}
\def\ordalsq {{\ensuremath{\mathcal{O}(\alpha^{2})}}\xspace}
\def\ordalcb {{\ensuremath{\mathcal{O}(\alpha^{3})}}\xspace}

%% QCD parameters
\newcommand{\as}{{\ensuremath{\alpha_s}}\xspace}
\newcommand{\MSb}{{\ensuremath{\overline{\mathrm{MS}}}}\xspace}
\newcommand{\lqcd}{{\ensuremath{\Lambda_{\mathrm{QCD}}}}\xspace}
\def\qsq       {{\ensuremath{q^2}}\xspace}

%% CKM, CP violation

\def\eps   {{\ensuremath{\varepsilon}}\xspace}
\def\epsK  {{\ensuremath{\varepsilon_K}}\xspace}
\def\epsB  {{\ensuremath{\varepsilon_B}}\xspace}
\def\epsp  {{\ensuremath{\varepsilon^\prime_K}}\xspace}

\def\CP                {{\ensuremath{C\!P}}\xspace}
\def\CPT               {{\ensuremath{C\!PT}}\xspace}

\def\rhobar {{\ensuremath{\overline \rho}}\xspace}
\def\etabar {{\ensuremath{\overline \eta}}\xspace}

\def\Vud  {{\ensuremath{V_{\uquark\dquark}}}\xspace}
\def\Vcd  {{\ensuremath{V_{\cquark\dquark}}}\xspace}
\def\Vtd  {{\ensuremath{V_{\tquark\dquark}}}\xspace}
\def\Vus  {{\ensuremath{V_{\uquark\squark}}}\xspace}
\def\Vcs  {{\ensuremath{V_{\cquark\squark}}}\xspace}
\def\Vts  {{\ensuremath{V_{\tquark\squark}}}\xspace}
\def\Vub  {{\ensuremath{V_{\uquark\bquark}}}\xspace}
\def\Vcb  {{\ensuremath{V_{\cquark\bquark}}}\xspace}
\def\Vtb  {{\ensuremath{V_{\tquark\bquark}}}\xspace}
\def\Vuds  {{\ensuremath{V_{\uquark\dquark}^\ast}}\xspace}
\def\Vcds  {{\ensuremath{V_{\cquark\dquark}^\ast}}\xspace}
\def\Vtds  {{\ensuremath{V_{\tquark\dquark}^\ast}}\xspace}
\def\Vuss  {{\ensuremath{V_{\uquark\squark}^\ast}}\xspace}
\def\Vcss  {{\ensuremath{V_{\cquark\squark}^\ast}}\xspace}
\def\Vtss  {{\ensuremath{V_{\tquark\squark}^\ast}}\xspace}
\def\Vubs  {{\ensuremath{V_{\uquark\bquark}^\ast}}\xspace}
\def\Vcbs  {{\ensuremath{V_{\cquark\bquark}^\ast}}\xspace}
\def\Vtbs  {{\ensuremath{V_{\tquark\bquark}^\ast}}\xspace}

%% Oscillations

\newcommand{\dm}{{\ensuremath{\Delta m}}\xspace}
\newcommand{\dms}{{\ensuremath{\Delta m_{\squark}}}\xspace}
\newcommand{\dmd}{{\ensuremath{\Delta m_{\dquark}}}\xspace}
\newcommand{\DG}{{\ensuremath{\Delta\Gamma}}\xspace}
\newcommand{\DGs}{{\ensuremath{\Delta\Gamma_{\squark}}}\xspace}
\newcommand{\DGd}{{\ensuremath{\Delta\Gamma_{\dquark}}}\xspace}
\newcommand{\Gs}{{\ensuremath{\Gamma_{\squark}}}\xspace}
\newcommand{\Gd}{{\ensuremath{\Gamma_{\dquark}}}\xspace}
\newcommand{\MBq}{{\ensuremath{M_{\B_\quark}}}\xspace}
\newcommand{\DGq}{{\ensuremath{\Delta\Gamma_{\quark}}}\xspace}
\newcommand{\Gq}{{\ensuremath{\Gamma_{\quark}}}\xspace}
\newcommand{\dmq}{{\ensuremath{\Delta m_{\quark}}}\xspace}
\newcommand{\GL}{{\ensuremath{\Gamma_{\mathrm{ L}}}}\xspace}
\newcommand{\GH}{{\ensuremath{\Gamma_{\mathrm{ H}}}}\xspace}
\newcommand{\DGsGs}{{\ensuremath{\Delta\Gamma_{\squark}/\Gamma_{\squark}}}\xspace}
\newcommand{\Delm}{{\mbox{$\Delta m $}}\xspace}
\newcommand{\ACP}{{\ensuremath{{\mathcal{A}}^{\CP}}}\xspace}
\newcommand{\Adir}{{\ensuremath{{\mathcal{A}}^{\mathrm{ dir}}}}\xspace}
\newcommand{\Amix}{{\ensuremath{{\mathcal{A}}^{\mathrm{ mix}}}}\xspace}
\newcommand{\ADelta}{{\ensuremath{{\mathcal{A}}^\Delta}}\xspace}
\newcommand{\phid}{{\ensuremath{\phi_{\dquark}}}\xspace}
\newcommand{\sinphid}{{\ensuremath{\sin\!\phid}}\xspace}
\newcommand{\phis}{{\ensuremath{\phi_{\squark}}}\xspace}
\newcommand{\betas}{{\ensuremath{\beta_{\squark}}}\xspace}
\newcommand{\sbetas}{{\ensuremath{\sigma(\beta_{\squark})}}\xspace}
\newcommand{\stbetas}{{\ensuremath{\sigma(2\beta_{\squark})}}\xspace}
\newcommand{\stphis}{{\ensuremath{\sigma(\phi_{\squark})}}\xspace}
\newcommand{\sinphis}{{\ensuremath{\sin\!\phis}}\xspace}

%% Tagging
\newcommand{\edet}{{\ensuremath{\varepsilon_{\mathrm{ det}}}}\xspace}
\newcommand{\erec}{{\ensuremath{\varepsilon_{\mathrm{ rec/det}}}}\xspace}
\newcommand{\esel}{{\ensuremath{\varepsilon_{\mathrm{ sel/rec}}}}\xspace}
\newcommand{\etrg}{{\ensuremath{\varepsilon_{\mathrm{ trg/sel}}}}\xspace}
\newcommand{\etot}{{\ensuremath{\varepsilon_{\mathrm{ tot}}}}\xspace}

\newcommand{\mistag}{\ensuremath{\omega}\xspace}
\newcommand{\wcomb}{\ensuremath{\omega^{\mathrm{comb}}}\xspace}
\newcommand{\etag}{{\ensuremath{\varepsilon_{\mathrm{tag}}}}\xspace}
\newcommand{\etagcomb}{{\ensuremath{\varepsilon_{\mathrm{tag}}^{\mathrm{comb}}}}\xspace}
\newcommand{\effeff}{\ensuremath{\varepsilon_{\mathrm{eff}}}\xspace}
\newcommand{\effeffcomb}{\ensuremath{\varepsilon_{\mathrm{eff}}^{\mathrm{comb}}}\xspace}
\newcommand{\efftag}{{\ensuremath{\etag(1-2\omega)^2}}\xspace}
\newcommand{\effD}{{\ensuremath{\etag D^2}}\xspace}

\newcommand{\etagprompt}{{\ensuremath{\varepsilon_{\mathrm{ tag}}^{\mathrm{Pr}}}}\xspace}
\newcommand{\etagLL}{{\ensuremath{\varepsilon_{\mathrm{ tag}}^{\mathrm{LL}}}}\xspace}

%% Key decay channels

\def\BdToKstmm    {\decay{\Bd}{\Kstarz\mup\mun}}
\def\BdbToKstmm   {\decay{\Bdb}{\Kstarzb\mup\mun}}

\def\BsToJPsiPhi  {\decay{\Bs}{\jpsi\phi}}
\def\BdToJPsiKst  {\decay{\Bd}{\jpsi\Kstarz}}
\def\BdbToJPsiKst {\decay{\Bdb}{\jpsi\Kstarzb}}

\def\BsPhiGam     {\decay{\Bs}{\phi \g}}
\def\BdKstGam     {\decay{\Bd}{\Kstarz \g}}

\def\BTohh        {\decay{\B}{\Ph^+ \Ph'^-}}
\def\BdTopipi     {\decay{\Bd}{\pip\pim}}
\def\BdToKpi      {\decay{\Bd}{\Kp\pim}}
\def\BsToKK       {\decay{\Bs}{\Kp\Km}}
\def\BsTopiK      {\decay{\Bs}{\pip\Km}}

%% Rare decays
\def\BdKstee  {\decay{\Bd}{\Kstarz\epem}}
\def\BdbKstee {\decay{\Bdb}{\Kstarzb\epem}}
\def\bsll     {\decay{\bquark}{\squark \ell^+ \ell^-}}
\def\AFB      {\ensuremath{A_{\mathrm{FB}}}\xspace}
\def\FL       {\ensuremath{F_{\mathrm{L}}}\xspace}
\def\AT#1     {\ensuremath{A_{\mathrm{T}}^{#1}}\xspace}           % 2
\def\btosgam  {\decay{\bquark}{\squark \g}}
\def\btodgam  {\decay{\bquark}{\dquark \g}}
\def\Bsmm     {\decay{\Bs}{\mup\mun}}
\def\Bdmm     {\decay{\Bd}{\mup\mun}}
\def\ctl       {\ensuremath{\cos{\theta_\ell}}\xspace}
\def\ctk       {\ensuremath{\cos{\theta_K}}\xspace}

%% Wilson coefficients and operators
\def\C#1      {\ensuremath{\mathcal{C}_{#1}}\xspace}                       % 9
\def\Cp#1     {\ensuremath{\mathcal{C}_{#1}^{'}}\xspace}                    % 7
\def\Ceff#1   {\ensuremath{\mathcal{C}_{#1}^{\mathrm{(eff)}}}\xspace}        % 9  
\def\Cpeff#1  {\ensuremath{\mathcal{C}_{#1}^{'\mathrm{(eff)}}}\xspace}       % 7
\def\Ope#1    {\ensuremath{\mathcal{O}_{#1}}\xspace}                       % 2
\def\Opep#1   {\ensuremath{\mathcal{O}_{#1}^{'}}\xspace}                    % 7

%% Charm

\def\xprime     {\ensuremath{x^{\prime}}\xspace}
\def\yprime     {\ensuremath{y^{\prime}}\xspace}
\def\ycp        {\ensuremath{y_{\CP}}\xspace}
\def\agamma     {\ensuremath{A_{\Gamma}}\xspace}
%%%\def\kpi        {\ensuremath{\PK\Ppi}\xspace}
%%%\def\kk         {\ensuremath{\PK\PK}\xspace}
%%%\def\dkpi       {\decay{\PD}{\PK\Ppi}}
%%%\def\dkk        {\decay{\PD}{\PK\PK}}
\def\dkpicf     {\decay{\Dz}{\Km\pip}}

%% QM
\newcommand{\bra}[1]{\ensuremath{\langle #1|}}             % {a}
\newcommand{\ket}[1]{\ensuremath{|#1\rangle}}              % {b}
\newcommand{\braket}[2]{\ensuremath{\langle #1|#2\rangle}} % {a}{b}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Units
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\unit}[1]{\ensuremath{\mathrm{ \,#1}}\xspace}          % {kg}

%% Energy and momentum
\newcommand{\tev}{\ifthenelse{\boolean{inbibliography}}{\ensuremath{~T\kern -0.05em eV}\xspace}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\gevgevcccc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V^2\!/}c^4}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}

%% Distance and area
\def\km   {\ensuremath{\mathrm{ \,km}}\xspace}
\def\m    {\ensuremath{\mathrm{ \,m}}\xspace}
\def\ma   {\ensuremath{{\mathrm{ \,m}}^2}\xspace}
\def\cm   {\ensuremath{\mathrm{ \,cm}}\xspace}
\def\cma  {\ensuremath{{\mathrm{ \,cm}}^2}\xspace}
\def\mm   {\ensuremath{\mathrm{ \,mm}}\xspace}
\def\mma  {\ensuremath{{\mathrm{ \,mm}}^2}\xspace}
\def\mum  {\ensuremath{{\,\upmu\mathrm{m}}}\xspace}
\def\muma {\ensuremath{{\,\upmu\mathrm{m}^2}}\xspace}
\def\nm   {\ensuremath{\mathrm{ \,nm}}\xspace}
\def\fm   {\ensuremath{\mathrm{ \,fm}}\xspace}
\def\barn{\ensuremath{\mathrm{ \,b}}\xspace}
%%%\def\barnhyph{\ensuremath{\mathrm{ -b}}\xspace}
\def\mbarn{\ensuremath{\mathrm{ \,mb}}\xspace}
\def\mub{\ensuremath{{\mathrm{ \,\upmu b}}}\xspace}
%%%\def\mbarnhyph{\ensuremath{\mathrm{ -mb}}\xspace}
\def\nb {\ensuremath{\mathrm{ \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{\mathrm{ \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}

%% Time 
\def\sec  {\ensuremath{\mathrm{{\,s}}}\xspace}
\def\ms   {\ensuremath{{\mathrm{ \,ms}}}\xspace}
\def\mus  {\ensuremath{{\,\upmu{\mathrm{ s}}}}\xspace}
\def\ns   {\ensuremath{{\mathrm{ \,ns}}}\xspace}
\def\ps   {\ensuremath{{\mathrm{ \,ps}}}\xspace}
\def\fs   {\ensuremath{\mathrm{ \,fs}}\xspace}

\def\mhz  {\ensuremath{{\mathrm{ \,MHz}}}\xspace}
\def\khz  {\ensuremath{{\mathrm{ \,kHz}}}\xspace}
\def\hz   {\ensuremath{{\mathrm{ \,Hz}}}\xspace}

\def\invps{\ensuremath{{\mathrm{ \,ps^{-1}}}}\xspace}
\def\invns{\ensuremath{{\mathrm{ \,ns^{-1}}}}\xspace}

\def\yr   {\ensuremath{\mathrm{ \,yr}}\xspace}
\def\hr   {\ensuremath{\mathrm{ \,hr}}\xspace}

%% Temperature
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\mathrm{ K}}\xspace}

%% Material lengths, radiation
\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\def\mip {MIP\xspace}
\def\neutroneq {\ensuremath{\mathrm{ \,n_{eq}}}\xspace}
\def\neqcmcm {\ensuremath{\mathrm{ \,n_{eq} / cm^2}}\xspace}
\def\kRad {\ensuremath{\mathrm{ \,kRad}}\xspace}
\def\MRad {\ensuremath{\mathrm{ \,MRad}}\xspace}
\def\ci {\ensuremath{\mathrm{ \,Ci}}\xspace}
\def\mci {\ensuremath{\mathrm{ \,mCi}}\xspace}

%% Uncertainties
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    

\newcommand{\stat}{\ensuremath{\mathrm{\,(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{\,(syst)}}\xspace}

%% Maths

\def\order{{\ensuremath{\mathcal{O}}}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\chisqndf}{\ensuremath{\chi^2/\mathrm{ndf}}\xspace}
\newcommand{\chisqip}{\ensuremath{\chi^2_{\text{IP}}}\xspace}
\newcommand{\chisqvs}{\ensuremath{\chi^2_{\text{VS}}}\xspace}
\newcommand{\chisqvtx}{\ensuremath{\chi^2_{\text{vtx}}}\xspace}
\newcommand{\chisqvtxndf}{\ensuremath{\chi^2_{\text{vtx}}/\mathrm{ndf}}\xspace}

\def\deriv {\ensuremath{\mathrm{d}}}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\newcommand{\mean}[1]{\ensuremath{\left\langle #1 \right\rangle}} % {x}
\newcommand{\abs}[1]{\ensuremath{\left\|#1\right\|}} % {x}
\newcommand{\Real}{\ensuremath{\mathcal{R}e}\xspace}
\newcommand{\Imag}{\ensuremath{\mathcal{I}m}\xspace}

\def\PDF {PDF\xspace}

\def\sPlot{\mbox{\em sPlot}\xspace}
%%%\def\sWeight{\mbox{\em sWeight}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Kinematics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Energy, Momenta
\def\Ebeam {\ensuremath{E_{\mbox{\tiny BEAM}}}\xspace}
\def\sqs   {\ensuremath{\protect\sqrt{s}}\xspace}

\def\ptot       {\mbox{$p$}\xspace}
\def\pt         {\mbox{$p_{\mathrm{ T}}$}\xspace}
\def\et         {\mbox{$E_{\mathrm{ T}}$}\xspace}
\def\mt         {\mbox{$M_{\mathrm{ T}}$}\xspace}
\def\dpp        {\ensuremath{\Delta p/p}\xspace}
\def\msq        {\ensuremath{m^2}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}

%% PID

\def\dllkpi     {\ensuremath{\mathrm{DLL}_{\kaon\pion}}\xspace}
\def\dllppi     {\ensuremath{\mathrm{DLL}_{\proton\pion}}\xspace}
\def\dllepi     {\ensuremath{\mathrm{DLL}_{\electron\pion}}\xspace}
\def\dllmupi    {\ensuremath{\mathrm{DLL}_{\muon\pi}}\xspace}

%% Geometry
%%%\def\mphi       {\mbox{$\phi$}\xspace}
%%%\def\mtheta     {\mbox{$\theta$}\xspace}
%%%\def\ctheta     {\mbox{$\cos\theta$}\xspace}
%%%\def\stheta     {\mbox{$\sin\theta$}\xspace}
%%%\def\ttheta     {\mbox{$\tan\theta$}\xspace}

\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\krad {\ensuremath{\mathrm{ \,krad}}\xspace}
\def\mrad{\ensuremath{\mathrm{ \,mrad}}\xspace}
\def\rad{\ensuremath{\mathrm{ \,rad}}\xspace}

%% Accelerator
\def\betastar {\ensuremath{\beta^*}}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}
\newcommand{\intlum}[1]{\ensuremath{\int\lum=#1}\xspace}  % {2 \,\invfb}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Software
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Programs
%%%\def\ansys      {\mbox{\textsc{Ansys}}\xspace}
\def\bcvegpy    {\mbox{\textsc{Bcvegpy}}\xspace}
\def\boole      {\mbox{\textsc{Boole}}\xspace}
\def\brunel     {\mbox{\textsc{Brunel}}\xspace}
\def\davinci    {\mbox{\textsc{DaVinci}}\xspace}
\def\dirac      {\mbox{\textsc{Dirac}}\xspace}
%%%\def\erasmus    {\mbox{\textsc{Erasmus}}\xspace}
\def\evtgen     {\mbox{\textsc{EvtGen}}\xspace}
\def\fewz       {\mbox{\textsc{Fewz}}\xspace}
\def\fluka      {\mbox{\textsc{Fluka}}\xspace}
\def\ganga      {\mbox{\textsc{Ganga}}\xspace}
%%%\def\garfield   {\mbox{\textsc{Garfield}}\xspace}
\def\gaudi      {\mbox{\textsc{Gaudi}}\xspace}
\def\gauss      {\mbox{\textsc{Gauss}}\xspace}
\def\geant      {\mbox{\textsc{Geant4}}\xspace}
\def\hepmc      {\mbox{\textsc{HepMC}}\xspace}
\def\herwig     {\mbox{\textsc{Herwig}}\xspace}
\def\moore      {\mbox{\textsc{Moore}}\xspace}
\def\neurobayes {\mbox{\textsc{NeuroBayes}}\xspace}
\def\photos     {\mbox{\textsc{Photos}}\xspace}
\def\powheg     {\mbox{\textsc{Powheg}}\xspace}
%%%\def\pyroot     {\mbox{\textsc{PyRoot}}\xspace}
\def\pythia     {\mbox{\textsc{Pythia}}\xspace}
\def\resbos     {\mbox{\textsc{ResBos}}\xspace}
\def\roofit     {\mbox{\textsc{RooFit}}\xspace}
\def\root       {\mbox{\textsc{Root}}\xspace}
\def\spice      {\mbox{\textsc{Spice}}\xspace}
%%%\def\tosca      {\mbox{\textsc{Tosca}}\xspace}
\def\urania     {\mbox{\textsc{Urania}}\xspace}

%% Languages
\def\cpp        {\mbox{\textsc{C\raisebox{0.1em}{{\footnotesize{++}}}}}\xspace}
%%%\def\python     {\mbox{\textsc{Python}}\xspace}
\def\ruby       {\mbox{\textsc{Ruby}}\xspace}
\def\fortran    {\mbox{\textsc{Fortran}}\xspace}
\def\svn        {\mbox{\textsc{SVN}}\xspace}

%% Data processing
\def\kbytes     {\ensuremath{{\mathrm{ \,kbytes}}}\xspace}
\def\kbsps      {\ensuremath{{\mathrm{ \,kbytes/s}}}\xspace}
\def\kbits      {\ensuremath{{\mathrm{ \,kbits}}}\xspace}
\def\kbsps      {\ensuremath{{\mathrm{ \,kbits/s}}}\xspace}
\def\mbsps      {\ensuremath{{\mathrm{ \,Mbits/s}}}\xspace}
\def\mbytes     {\ensuremath{{\mathrm{ \,Mbytes}}}\xspace}
\def\mbps       {\ensuremath{{\mathrm{ \,Mbyte/s}}}\xspace}
\def\mbsps      {\ensuremath{{\mathrm{ \,Mbytes/s}}}\xspace}
\def\gbsps      {\ensuremath{{\mathrm{ \,Gbits/s}}}\xspace}
\def\gbytes     {\ensuremath{{\mathrm{ \,Gbytes}}}\xspace}
\def\gbsps      {\ensuremath{{\mathrm{ \,Gbytes/s}}}\xspace}
\def\tbytes     {\ensuremath{{\mathrm{ \,Tbytes}}}\xspace}
\def\tbpy       {\ensuremath{{\mathrm{ \,Tbytes/yr}}}\xspace}

\def\dst        {DST\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Detector related
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Detector technologies
\def\nonn {\ensuremath{\mathrm{{ \mathit{n^+}} \mbox{-} on\mbox{-}{ \mathit{n}}}}\xspace}
\def\ponn {\ensuremath{\mathrm{{ \mathit{p^+}} \mbox{-} on\mbox{-}{ \mathit{n}}}}\xspace}
\def\nonp {\ensuremath{\mathrm{{ \mathit{n^+}} \mbox{-} on\mbox{-}{ \mathit{p}}}}\xspace}
\def\cvd  {CVD\xspace}
\def\mwpc {MWPC\xspace}
\def\gem  {GEM\xspace}

%% Detector components, electronics
\def\tell1  {TELL1\xspace}
\def\ukl1   {UKL1\xspace}
\def\beetle {Beetle\xspace}
\def\otis   {OTIS\xspace}
\def\croc   {CROC\xspace}
\def\carioca {CARIOCA\xspace}
\def\dialog {DIALOG\xspace}
\def\sync   {SYNC\xspace}
\def\cardiac {CARDIAC\xspace}
\def\gol    {GOL\xspace}
\def\vcsel  {VCSEL\xspace}
\def\ttc    {TTC\xspace}
\def\ttcrx  {TTCrx\xspace}
\def\hpd    {HPD\xspace}
\def\pmt    {PMT\xspace}
\def\specs  {SPECS\xspace}
\def\elmb   {ELMB\xspace}
\def\fpga   {FPGA\xspace}
\def\plc    {PLC\xspace}
\def\rasnik {RASNIK\xspace}
\def\elmb   {ELMB\xspace}
\def\can    {CAN\xspace}
\def\lvds   {LVDS\xspace}
\def\ntc    {NTC\xspace}
\def\adc    {ADC\xspace}
\def\led    {LED\xspace}
\def\ccd    {CCD\xspace}
\def\hv     {HV\xspace}
\def\lv     {LV\xspace}
\def\pvss   {PVSS\xspace}
\def\cmos   {CMOS\xspace}
\def\fifo   {FIFO\xspace}
\def\ccpc   {CCPC\xspace}

%% Chemical symbols
\def\cfourften     {\ensuremath{\mathrm{ C_4 F_{10}}}\xspace}
\def\cffour        {\ensuremath{\mathrm{ CF_4}}\xspace}
\def\cotwo         {\ensuremath{\mathrm{ CO_2}}\xspace} 
\def\csixffouteen  {\ensuremath{\mathrm{ C_6 F_{14}}}\xspace} 
\def\mgftwo     {\ensuremath{\mathrm{ Mg F_2}}\xspace} 
\def\siotwo     {\ensuremath{\mathrm{ SiO_2}}\xspace} 

%%%%%%%%%%%%%%%
% Special Text 
%%%%%%%%%%%%%%%
\newcommand{\eg}{\mbox{\itshape e.g.}\xspace}
\newcommand{\ie}{\mbox{\itshape i.e.}\xspace}
\newcommand{\etal}{\mbox{\itshape et al.}\xspace}
\newcommand{\etc}{\mbox{\itshape etc.}\xspace}
\newcommand{\cf}{\mbox{\itshape cf.}\xspace}
\newcommand{\ffp}{\mbox{\itshape ff.}\xspace}
\newcommand{\vs}{\mbox{\itshape vs.}\xspace}


==> sections/vertex_characterisation.tex <==
\section{Results of single runs}

Here we report results from all the runs included in the analysis reported in this document (see Table \ref{tab:eff}).

The reconstructed position of interaction-vertex candidates along the beam direction is shown in Figures~\ref{fig:charm_primaryZ1}, \ref{fig:charm_primaryZ2} and \ref{fig:charm_primaryZ3}. Data and Monte Carlo distributions have been normalised to the number of p.o.t. integrated in each run.

The interaction vertex multiplicity for different runs is reported in Figures~\ref{fig:charm_primaryvertex1}, \ref{fig:charm_primaryvertex2} and  \ref{fig:charm_primaryvertex3}. The contribution of the primary proton and hadron-reinteraction components is shown separately. Data and Monte Carlo distributions have been normalised to the number of p.o.t. integrated in each run.

\begin{figure}[htbp]
\centering
\includegraphics[scale=0.38]{figs/CH1_vz_part.png}
\caption{Vertex position along the beam direction for interaction-vertex candidates reconstructed four runs of configuration CHARM1.}
\label{fig:charm_primaryZ1}
\end{figure}%

\begin{figure}[htbp]
\centering
\includegraphics[width=1.0\linewidth]{figs/CH2_vz_part.png}
\caption{Vertex position along the beam direction for interaction-vertex candidates reconstructed three runs of configuration CHARM2.}
\label{fig:charm_primaryZ2}
\end{figure}%

\begin{figure}[htbp]
\centering
\includegraphics[width=1.0\linewidth]{figs/CH3_vz_part.png}
\caption{Vertex position along the beam direction for interaction-vertex candidates reconstructed in the first run of configurations CHARM3, CHARM4, CHARM5 and CHARM6.}
\label{fig:charm_primaryZ3}
\end{figure}%


\begin{figure}[htbp]
\centering
\includegraphics[width=1.0\linewidth]{figs/CH1_mult_part.png}
\caption{Charged track multiplicity for interaction-vertex candidates reconstructed in four runs of configuration CHARM1.}
\label{fig:charm_primaryvertex1}
\end{figure}%

\begin{figure}[htbp]
\centering
\includegraphics[width=1.0\linewidth]{figs/CH2_mult_part.png}
\caption{Charged track multiplicity for interaction-vertex candidates reconstructed three runs of configuration CHARM2.}
\label{fig:charm_primaryvertex2}
\end{figure}%

\begin{figure}[htbp]
\centering
\includegraphics[width=1.0\linewidth]{figs/CH3_mult_part.png}
\caption{Charged track multiplicity for interaction-vertex candidates reconstructed in the first run of configurations CHARM3, CHARM4, CHARM5 and CHARM6.}
\label{fig:charm_primaryvertex3}
\end{figure}%

